Scalable Methods for Brick Kiln Detection and Compliance Monitoring from Satellite Imagery: A Deployment Case Study in India

Air pollution kills 7 million people annually. Brick manufacturing industry is the second largest consumer of coal contributing to 8%-14% of air pollution in Indo-Gangetic plain (highly populated tract of land in the Indian subcontinent). As brick kilns are an unorganized sector and present in large numbers, detecting policy violations such as distance from habitat is non-trivial. Air quality and other domain experts rely on manual human annotation to maintain brick kiln inventory. Previous work used computer vision based machine learning methods to detect brick kilns from satellite imagery but they are limited to certain geographies and labeling the data is laborious. In this paper, we propose a framework to deploy a scalable brick kiln detection system for large countries such as India and identify 7477 new brick kilns from 28 districts in 5 states in the Indo-Gangetic plain. We then showcase efficient ways to check policy violations such as high spatial density of kilns and abnormal increase over time in a region. We show that 90% of brick kilns in Delhi-NCR violate a density-based policy. Our framework can be directly adopted by the governments across the world to automate the policy regulations around brick kilns.

==> background.tex <==
% \section{Background}

% \subsection{Binary Image Classification with Machine Learning}
% ...

==> baseline_approach.tex <==
We compare our method with the approach described in \cite{lee2021scalable} and other standard methods used in previous studies. We tested various convolutional neural network models like the vision transformer\cite{dosovitskiy2020image}, VGG16\cite{simonyan2014very}, and ResNet50\cite{he2016deep}. However, due to space constraints, we do not provide detailed comparisons here. It's important to note that the results from these models were similar to or worse than the benchmarks mentioned in prior research.\\
\\
\textbf{ResNet50:} ResNet50 is a commonly utilized architecture known for its effectiveness in image classification tasks \cite{he2016deep}. Its key feature lies in the implementation of residual connections, which enable deeper networks to be trained more effectively by mitigating the vanishing gradient problem and facilitating the flow of information through the network.\\
\\
\textbf{EfficientNetB0:} EfficientNetB0 is a highly regarded architecture acknowledged for its remarkable performance in image classification tasks \cite{tan2019efficientnet}. Its distinguishing feature lies in its efficient scaling of network depth, width, and resolution, achieving impressive accuracy with significantly fewer parameters compared to other models. This efficiency makes it particularly suitable for resource-constrained environments and mobile applications.\\
\\
\textbf{DenseNet121:} DenseNet121 is a widely recognized architecture notable for its dense connectivity patterns among layers \cite{huang2017densely}. Unlike traditional architectures, DenseNet forms direct connections between all layers, promoting feature reuse and enhancing gradient flow throughout the network. This dense connectivity contributes to improved model accuracy and parameter efficiency, making DenseNet121 an attractive choice for various image classification tasks.

